On a condition for type-I Bose-Einstein condensation in random potentials in $d$ dimensions

In this paper we discuss Bose-Einstein condensation (BEC) in systems of pairwise non-interacting bosons in random potentials in $d$ dimensions. Working in a rather general framework, we provide a "gap condition" which is sufficient to conclude existence of type-I BEC in probability and in the $r$th mean. We illustrate our results in the context of the well-known (one-dimensional) Luttinger-Sy model. Here, whenever the particle density exceeds a critical value, we show in addition that only the ground state is macroscopically occupied.

==> def2.tex <==

\usepackage[ngerman,american]{babel}
\usepackage[utf8]{inputenc}


\usepackage{mathrsfs}
%\renewcommand{\mathbb}{\mathds}

\usepackage{amsmath,amsthm,amssymb,latexsym,amsfonts,mathabx,amscd,bbm}%a4wide}

\usepackage{fancyhdr} %Für LMU Templet?
\usepackage{parskip} % Absatzpaket
\setlength{\parindent}{2em}
\setlength{\parskip}{0pt}
\usepackage{setspace}
\usepackage{float}
%\usepackage[top=2.1cm,left=2.8cm,right=3.3cm,bottom=3cm]{geometry} %für DinA4 format
%\usepackage[top=1.75cm,left=1.75cm,right=3.5cm,bottom=2.25cm]{geometry}
\usepackage[top=1in,left=2.25cm,right=3cm,bottom=1in]{geometry}
\setlength{\headheight}{26pt}
%\setlength{\headsep}{0.4in} %für DinA4 format
\setlength{\headsep}{0.35in}
%\setlength{\footskip}{1.3cm} %Für DinA4 wieder hin
%
%\usepackage[paperwidth=6in, paperheight=9in, top=0.5in, margin=1in]{geometry}
%\usepackage[paperwidth=8in, paperheight=9in, top=0.5in, left=1in, right=1in, bottom=1in,includehead]{geometry}
%\usepackage[top=0.5in, left=1in, right=1in, bottom=1in,includehead]{geometry}
%\renewcommand{\headrulewidth}{0pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{graphicx} % Einbinden von Grafiken
%\usepackage{color} % farbiger Text
%\usepackage[gen]{eurosym} % Eurosymbol
 \usepackage{mathtools}% lädt auch amsmath 
 %\usepackage{amsmath}
%\usepackage[intlimits]{amsmath} % Mathe-Paket
%\usepackage{amssymb} % stellt weitere Symbole
%\usepackage{amsfonts} % Mathe-Schriften
%\usepackage{amsthm} % Theorem-Paket
\usepackage{dsfont}
%\usepackage{bbm}
\usepackage{mathrsfs} 
%\usepackage{fixltx2e} % macht u.a. \(...\) und \[...\] robust
%\usepackage[ngerman=ngerman-x-latest]{hyphsubst}
%\usepackage{mathptmx} %Schrift
\usepackage{courier}
%\usepackage{lmodern}
%\usepackage{mathpazo}
%\usepackage[libertine,cmintegrals,cmbraces,vvarbb]{newtxmath}
\usepackage{enumerate}
\usepackage{extarrows}
\usepackage{bm}
%\usepackage[pdfstartview={FitH},colorlinks]{hyperref} 
%\usepackage{bibgerm,cite}       % Deutsche Bezeichnungen, Automatisches Zusammenfassen von Literaturstellen
\usepackage{framed}
%\usepackage{babelbib}

\usepackage{color}


%\usepackage{enumitem}


\usepackage{verbatim} %fuer \begin{comment}

%\usepackage{hyperref}
\usepackage[pdfstartview={FitH},colorlinks, linkcolor=black, citecolor=black]{hyperref} 

\usepackage{bm}

\usepackage{pdfpages}

%\usepackage{ntheorem}

\usepackage{lipsum}

\usepackage{longtable}

\usepackage{graphicx}
\usepackage{pdfpages}
%\usepackage{scrlayer-scrpage}
\usepackage{changes}
\usepackage{interval}



\hyphenation{IN-TE-RES-SANT IN-TE-RES-SAN-TE SEI-TEN-UM-BRUCH 	O-PER-A-TOR 
HIL-BERT-RAUM HA-MIL-TON-O-PER-A-TOR HA-MIL-TON-O-PER-A-TORS OR-THO-NOR-MAL-BA-SIS HA-MIL-TON-FUN-KTION 
BO-SON-QUA-TEN-SYS-TEMS BO-SE-EIN-STEIN-KON-DEN-SA-TION TEIL-CHEN-HAM-IL-TON-O-PER-A-TOR
N-TEIL-CHEN-HAM-IL-TON-O-PER-A-TORS Hamiltonoperators VIEL-TEIL-CHEN-HA-MIL-TON-O-PER-A-TORS
}

%---------------------------------------------------------------------

%Theorem-Umgebung von Hagen



  \usepackage{graphicx}
% \usepackage{german}
%\usepackage[bookmarks]{hyperref}
%\usepackage{amssymb}





\newcommand{\ud}{\mathrm{d}}
\newcommand{\ui}{\mathrm{i}}
\newcommand{\ue}{\mathrm{e}}
\newcommand{\dM}{\mathrm{dM}}
\newcommand{\dl}{\mathrm{d}\ell}
\newcommand{\TRd}{\mathrm{T}^*\rz^d}
\newcommand{\skl}{\mathrm{S}}
\newcommand{\scl}{\mathrm{S}_{\mathrm{cl}}}
\newcommand{\sinv}{\mathrm{S}_{\mathrm{inv}}}
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\M}{\mathrm{M}}
\newcommand{\SU}{\mathrm{SU}}
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\U}{\mathrm{U}}
\newcommand{\su}{\mathrm{su}}
\newcommand{\uu}{\mathrm{u}}
\newcommand{\Stwo}{\mathrm{S}^2}
\newcommand{\ds}{\displaystyle}

\newcommand{\e}{\mathrm{e}}

\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\newcommand{\eps}{\epsilon}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\la}{\lambda}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\si}{\sigma}
\newcommand{\Si}{\Sigma}

\newcommand{\vn}{\boldsymbol{n}}
\newcommand{\vp}{\boldsymbol{p}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\vw}{\boldsymbol{w}}
\newcommand{\vx}{\boldsymbol{x}}
\newcommand{\vy}{\boldsymbol{y}}
\newcommand{\vA}{\boldsymbol{A}}
\newcommand{\vB}{\boldsymbol{B}}
\newcommand{\vC}{\boldsymbol{C}}
\newcommand{\vE}{\boldsymbol{E}}
\newcommand{\vF}{\boldsymbol{F}}

\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vsigma}{\boldsymbol{\sigma}}
\newcommand{\vxi}{\boldsymbol{\xi}}

\newcommand{\cB}{{\hat B}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cL}{{\hat L}}
\newcommand{\cM}{{\hat M}}
\newcommand{\cP}{{\mathcal P}} 
\newcommand{\tcP}{\tilde {\hat  P}} 
\newcommand{\cS}{{\hat S}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cO}{{\hat O}}
\newcommand{\cQ}{{\hat Q}}
\newcommand{\cR}{{\hat R}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cX}{{\hat X}}



\newcommand{\gz}{{\mathbb Z}}
\newcommand{\rz}{{\mathbb R}}
\newcommand{\nz}{{\mathbb N}}
\newcommand{\kz}{{\mathbb C}}

\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\mtr}{tr}
\DeclareMathOperator{\vol}{vol}        
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\op}{op}
\DeclareMathOperator{\symb}{symb}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\rank}{rk}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\ts}{T}
\DeclareMathOperator{\aut}{aut}
\DeclareMathOperator{\inn}{I}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\diag}{diag}

\newcommand{\measure}{\mathscr M}


\newcommand{\dpr}{\partial}  
\newcommand{\mat}{\mathrm{M}} 
\newcommand{\Hf}{H_{\mathrm{free}}}
\newcommand{\hHf}{\hat{H}_{\mathrm{free}}}
\newcommand{\symbSW}{\symb^\mathrm{SW}}

\newcommand{\mtiny}[1]{\text{\tiny\ensuremath{#1}}}  
\newcommand{\bem}[1]{\footnote{\texttt{#1}}}

%\newcommand{\eins}{\mathmybb{1}}
\newcommand{\eins}{\mathds{1}}

\newtheoremstyle{normal}% normale Schrift
  {10pt}% hSpace abovei
  {10pt}% hSpace belowi6
  {\normalfont}% hBody fonti
  {}% hIndent amounti1
  {\bfseries}% hTheorem head fonti
  {}% Punctuation after theorem headi
  {0.8em}% hSpace after theorem headi2
  {\bfseries{\thmname{#1}\thmnumber{ #2}.\thmnote{ \hspace{0.5em}(#3)\newline}}
}
 
\newtheoremstyle{kursiv}% kursive Schrift	``
  {10pt}% hSpace abovei
  {10pt}% hSpace belowi
  {\itshape}% hBody fonti
  {}% hIndent amounti1
  {\bfseries}% hTheorem head fonti
  {}% Punctuation after theorem headi
  {0.8em}% hSpace after theorem headi2
  %{}% hTheorem head spec (can be left empty, meaning `normal')
  {\bfseries{\thmname{#1}\thmnumber{ #2}.\thmnote{ \hspace{0.5em}(#3)\newline}}
}

 \numberwithin{equation}{section}
 
\theoremstyle{normal}
  \newtheorem{definition}[subsection]{Definition}
  \newtheorem{bemerkung}[subsection]{Bemerkung}
  \newtheorem{erinnerung}[subsection]{Erinnerung}
  \newtheorem{beispiel}[subsection]{Example}
  \newtheorem{lemma}[subsection]{Lemma}
 
\theoremstyle{kursiv}
  \newtheorem{satz}[subsection]{Theorem}
  \newtheorem{kor}[subsection]{Corollary}
  \newtheorem{defundsatz}[subsection]{Definition and Theorem}
  \newtheorem{voraussetzung}[subsection]{Assumptions}
  \newtheorem{remark}[subsection]{Remark}
  \newtheorem{remarks}[subsection]{Remarks}
        
\begin{comment}
\newcommand{\laplace}{- \mathop{}\!\mathbin\bigtriangleup}
  \newcommand{\Dlaplace}[1]{\laplace_{#1}^D}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmk}{\bm{k}}
  \newcommand{\bmxp}{\bmx^{\perp}}
  \newcommand{\bmX}[1]{\bmx_{#1}^{\omega}}
\newcommand{\braket}[2]{\left\langle \left. \, #1\, \right| \,#2 \, \right\rangle}  
%\newcommand{\braketop}[3]{\, \left\langle #1 \, \right|\, #2 \, \left|\,  #3 \,\right\rangle}
 \newcommand{\braketop}[3]{\,  \left\langle #1 \, \left| \, #2 \, \right| \, #3 \, \right\rangle}
\newcommand{\hil}{\mathscr{H}}
\newcommand{\E}{\mathds{E}}
  \newcommand{\Var}{\mathrm{Var}} 
   \newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\ket}[1]{|\, #1 \, \rangle}  
%\newcommand{\skalar}[2]{\langle #1, #2 \rangle}
\newcommand{\Lambdap}{\Lambda_N^{\parallel}}
\newcommand{\Lambdas}{\Lambda_N^{\perp}}
\end{comment}
  
  
%-------------------------------------------------------------------------

\begin{comment}
\newcommand{\hMF}{\hamopein_N^{\text{MF}}}
\newcommand{\hMFjN}{\hamopein_N^{\text{MF},j}}
\newcommand{\hMFjgN}{\hamopein^{\text{MF}}(\lintv{p}, \gNpo)}
\newcommand{\hMFi}{\hamopein_{\text{MF}}^{\gamma_N^{p,\omega},(i)}}
%\newcommand{\hMFi}{\hamopein^{\text{MF},i}_N}
\newcommand{\hMFNgl}{\hamopein_N^{\text{MF}}(\gamma_N^{p,\omega})}
\newcommand{\hMFiomega}{\hamopein^{\text{MF}, i , \omega}_N}
\newcommand{\hMFomega}{\hamopein^{\text{MF}}_N}
\newcommand{\hMFiteTeilchen}{\hamopein^{\text{MF}, (i)}_{N}}
\newcommand{\hMFjteTeilchenNgo}{\hamopein^{\text{MF}, (j)}(\lintv{p}, N_N^p g_N)}
\newcommand{\hMFpNjteTeilchen}{\hamopein^{\text{MF}, p, (j)}_{N}}
\newcommand{\hamopein}{h}
\newcommand{\hamopN}{\hamop{N}}
\newcommand{\hamoptildeN}{\hamop{\widetilde N}}
\newcommand{\hamopNomega}{\hamop{N}^{\omega}}
\newcommand{\hamopNiomega}{H_{N}^{i,\omega}}
\newcommand{\hamopNjomega}{H_{N}^{j}}
\newcommand{\hamopeinL}{h_L}
\newcommand{\hamopL}{H_L}
\newcommand{\hamop}[1]{H_{#1}}
\newcommand{\hamopNganz}[1]{H^{\otimes #1}}
\newcommand{\sym}{\text{sym}}
\newcommand{\fock}{\mathcal F}
\newcommand{\fockL}{\mathcal F_L}
\newcommand{\fockH}{\fock(\hil)}
\newcommand{\fockN}{\bigoplus\limits_{N=0}^{\infty} \NTeilchenhil}
\newcommand{\fockHL}{\fockL(\hilL)}
\newcommand{\fockNL}{\bigoplus\limits_{N=0}^{\infty} \NTeilchenhil_L}
\newcommand{\focksymN}{\bigoplus\limits_{N=0}^{\infty} \NTeilchenhilsym}
\newcommand{\focksymtildeN}{\bigoplus\limits_{\widetilde N=0}^{\infty} \NtildeTeilchenhilsym}
\newcommand{\fockNskalar}[2]{\sum\limits_{N=0}^{\infty} \langle \,#1\, | \,#2\, 
\rangle_{\NTeilchenhil}}
\newcommand{\focksymNskalar}[2]{\sum\limits_{N=0}^{\infty} \langle \,#1\, | 
\,#2\, \rangle_{\NTeilchenhilsym}}
\newcommand{\skalarcd}{\langle \, \cdot \, | \, \cdot \, \rangle}
\newcommand{\fockNskalarcd}{\fockNskalar{\,\cdot\,}{\,\cdot\,}}
\newcommand{\focksymNskalarcd}{\focksymNskalar{\cdot}{\cdot}}
\newcommand{\fockNnorm}[1]{\|#1\|_{\fockN}}
\newcommand{\focksymNnorm}[1]{\|#1\|_{\focksymN}}
\newcommand{\fockNnormcd}{\|\,\cdot\,\|_{\fockN}}
\newcommand{\focksymNnormcd}{\|\,\cdot\,\|_{\focksymN}}
\newcommand{\fockhilNnorm}[1]{\sum\limits_{N=0}^{\infty} \hilNnorm{#1}^2}
\newcommand{\focksymhilNnorm}[1]{\sum\limits_{N=0}^{\infty} \hilNsymnorm{#1}^2}
\newcommand{\fockhilNnormw}[1]{\left(\sum\limits_{N=0}^{\infty} 
\hilNnorm{#1}^2 \right)^{\frac{1}{2}}}
\newcommand{\focksym}{\mathcal F_{\text{sym}}}
\newcommand{\focksymh}{\mathcal F_{\text{sym}}(\hil)}
\newcommand{\focksymskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\mathcal F_{\text{sym}}}}
\newcommand{\focksymskalarcd}{\focksymskalar{\cdot}{\cdot}}
\newcommand{\EinTeilchenhil}{\mathcal H^{(1)}}
\newcommand{\NTeilchenhil}{\mathcal H^{(N)}}
\newcommand{\NtildeTeilchenhil}{\mathcal H^{(\widetilde N)}}
\newcommand{\XTeilchenhil}[1]{\mathcal H^{(#1)}}
\newcommand{\XteilchenhilNp}[1]{\mathcal H^{(#1)}_{N,p}}
\newcommand{\XTeilchenhilomega}[1]{\mathcal H^{(#1),\omega}}
\newcommand{\XTeilchenhilsym}[1]{\mathcal H^{(#1)}_{\sym}}
\newcommand{\XTeilchenhilsymp}[1]{\mathcal H^{(#1)}_{N, p, \sym}}
\newcommand{\XTeilchenhilsymN}[1]{\mathcal H^{(#1)}_{N, \sym}}
\newcommand{\NTeilchenhilsym}{\NTeilchenhil_{\text{sym}}}
\newcommand{\NtildeTeilchenhilsym}{\NtildeTeilchenhil_{\text{sym}}}
\newcommand{\NTeilchenhilskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\NTeilchenhil}}
\newcommand{\XTeilchenhilskalar}[3]{\langle \, #2 \, | \, #3 \, 
\rangle_{\XTeilchenhil{#1}}}
\newcommand{\XTeilchenhilskalarcd}[1]{\langle \, \cdot \, | \, \cdot \, 
\rangle_{\XTeilchenhil{#1}}}
\newcommand{\XTeilchenhilnorm}[2]{ \| #2 \|_{\XTeilchenhil{#1}}}
\newcommand{\XTeilchenhilNsymorm}[2]{ \| #2 \|_{\XTeilchenhilsym{#1}}}
\newcommand{\NTeilchenhilsymskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\NTeilchenhilsym}}
\newcommand{\NtildeTeilchenhilsymskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\NtildeTeilchenhilsym}}
\newcommand{\NTeilchenhilskalarcd}{\NTeilchenhilskalar{\cdot}{\cdot}}
\newcommand{\NTeilchenhilsymskalarcd}{\NTeilchenhilsymskalar{\cdot}{\cdot}}
\newcommand{\NtildeTeilchenhilsymskalarcd}{\NtildeTeilchenhilsymskalar{\cdot}{\cdot}}
\newcommand{\Lskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{L^2(\mathds R^{Nd},\mathds C)}}
\newcommand{\Lskalarcd}{\Lskalar{\cdot}{\cdot}}
\newcommand{\NTeilchenhilnorm}[1]{\| #1 \|_{\NTeilchenhil}}
\newcommand{\NTeilchenhilnormcd}{\| \cdot \|_{\NTeilchenhil}}
\newcommand{\HsymN}{\mathscr{H}_{\text{sym}}^{(N)}}
\newcommand{\skalar}[2]{\langle #1, #2 \rangle}
\newcommand{\Nskalar}[2]{\sum\limits_{N=0}^{\infty} \langle 
        #1^{(N)} | #2^{(N)} \rangle_{\mathscr{H}_{\text{sym}}^{(N)}}}
\newcommand{\nskalar}[2]{\langle 
        #1^{(N)} | #2^{(N)} \rangle_{\mathscr{H}_{\text{sym}}^ {(N)}}}        
\newcommand{\fockskalar}[2]{\langle #1 | #2 \rangle_{\fock}}
\newcommand{\fockHskalar}[2]{\langle #1 | #2 \rangle_{\fockH}}
\newcommand{\focknorm}[1]{\|#1\|_{\fock}}
\newcommand{\EskalarZ}[2]{\langle #1 | #2 \rangle_{\mathcal E}}
\newcommand{\EskalarS}[6]{\langle #1 \otimes #2 \otimes \ldots \otimes #3, #4 
\otimes #5\otimes \ldots \otimes #6 \rangle_{\mathcal E}}
\newcommand{\Hskalar}[3]{\langle #1_{#3} | #2_{#3} \rangle_{\mathscr{H}_{#3}}}
%\newcommand{\hil}{\mathscr{H}}
\newcommand{\hilL}{\mathscr{H_L}}
\newcommand{\hilN}{\hil^{(N)}}
\newcommand{\hilNganz}{\hil^{\otimes N}}
\newcommand{\hilX}[1]{\hil_{#1}}
\newcommand{\hilNsym}{\hil^{(N)}_{\sym}}
\newcommand{\hilNtildesym}{\hil^{(\widetilde N)}_{\sym}}
\newcommand{\hilskalar}[2]{\langle \,#1\, | \,#2\, \rangle_{\hil}}
\newcommand{\hilskalarcd}{\hilskalar{\cdot}{\cdot}}
\newcommand{\hilNskalar}[2]{\langle \,#1\, | \,#2\, \rangle_{\hilN}}
\newcommand{\hilXskalar}[3]{\langle \,#1\, | \,#2\, \rangle_{\mathscr{H}_{#3}}}
\newcommand{\hilNsymskalar}[2]{\langle \, #1 \,  | \, #2 \, \rangle_{\hilNsym}}
\newcommand{\hilNskalarcd}{\hilNskalar{\,\cdot\,}{\,\cdot\,}}
\newcommand{\hilNsymskalarcd}{\hilNsymskalar{\,\cdot\,}{\,\cdot}}
\newcommand{\hilnorm}[1]{\|\, #1\, \|_{\hil}}
\newcommand{\hilNnorm}[1]{\|\, #1\, \|_{\hilN}}
\newcommand{\hilNsymnorm}[1]{\|\, #1\, \|_{\hilNsym}}
\newcommand{\bra}[1]{\langle \, #1 \, |}
%\newcommand{\ket}[1]{|\, #1 \, \rangle}
%\newcommand{\braket}[2]{\left\langle \left. \, #1\, \right| \,#2 \, \right\rangle}
%\newcommand{\braketop}[3]{\, \left\langle #1 \,|\, #2 \,|\, #3 \,\right\rangle}
%\newcommand{\braketop}[3]{\langle #1 |\, #2 \,| #3 \rangle}
\newcommand{\projec}[1]{\ket{#1}\bra{#1}}
\newcommand{\ONB}[1]{\left\{ \phi_{#1} \right\}_{#1 \in \mathds N}}
\newcommand{\ONBN}[1]{\left\{ \phi_{#1_1} \otimes \phi_{#1_2} \otimes \ldots \otimes \phi_{#1_N} \right\}_{#1_1, #1_2, \ldots, #1_N \in \mathds N}}

\newcommand{\gNpo}{N_N^p g_N}
\newcommand{\gNpotilde}{\widetilde g_N^{\,p}}
\newcommand{\gammaNpo}{\gamma_N^{\,p}}
\newcommand{\gammaNpotilde}{\widetilde \gamma_N^{\,p}}

\newcommand{\NNpGeord}[1]{N_{N,>}^{#1}}

\newcommand{\EQM}[1]{E_{\text{QM}}^{#1}\left( \widetilde N_N^p, \lintv{p}, g_N \right)}
\newcommand{\phiQM}[1]{\phi_N^{#1}}
\newcommand{\Hdimdrei}{H_{3D}(N,L,r,a)}
\newcommand{\br}[1]{b_r(\bm{x}^{\perp}_{#1})}
\newcommand{\Br}[1]{\prod\limits_{#1 = 1}^N \br{#1}}
\newcommand{\brquad}[1]{b_r^2(\bm{x}^{\perp}_{#1})}
\newcommand{\BrQuad}[1]{\prod\limits_{#1 = 1}^N \brquad{#1}}
\newcommand{\phigp}{\phi_{\text{GP}}}
\newcommand{\phigpgamma}{\phi_{\text{GP}}^{g_N}}
\newcommand{\phigpgNp}{\phi_{\text{GP}}(N_N^p, \lintv{p}, g_N)}
\newcommand{\phigpgeinsp}{\phi_{\text{GP}}(1, \lintv{p}, N_N^p g_N)}
\newcommand{\phigpgammap}{\phi_{\text{GP}}^{1, \gammaNpo}}
\newcommand{\phigpgNpo}{\phi_{\text{GP}}^{\lintv{p}, \gNpo}}
\newcommand{\phigpgammapeinslg}{\phi_{\text{GP}}(1, \lintv{p}, N_N^p g_N)}
\newcommand{\EGPgammaNpo}{\EGP ( 1, 1, \gammaNpo )}
\newcommand{\EGPgNpo}{\EGP(1, \lintv{p}, \gNpo)}
\newcommand{\phigpgammaptilde}{\widetilde\phi_{\text{GP}}^{\gammaNpo}}
\newcommand{\phigpgNpotilde}{\widetilde\phi_{\text{GP}}^{\, \lintv{p}, \gNpo}}
\newcommand{\phigpgammapl}{\phi_N^{\text{GP}}(\gamma_N^{p,\omega})}
\newcommand{\phigpgammaIp}{\phi_{\text{GP}, I^{p,\omega}}^{\gamma}}
\newcommand{\Kphigp}{\ket{\phi_{\text{GP}}}}
\newcommand{\Kphigpgamma}{\ket{\phi_N^{\text{GP}}}}
\newcommand{\Kphigpgammap}{\ket{\phi_{\text{GP}, I^{p,\omega}}^{\gamma}}}
\newcommand{\phigpN}{\phi_{\text{GP}}^{\otimes N}}
\newcommand{\phigpNjomega}{\left( \phigpgammap \right)^{\otimes N_N^p}}
\newcommand{\phiGP}[1]{\phi_{GP}(z_{#1})}
\newcommand{\phiGPL}[1]{\phi_{GP}\left( z_{#1}/L \right)}
\newcommand{\phiGPz}{\phi_{GP}(z)}
\newcommand{\phiGPzs}{\phi_{GP}(z')}
\newcommand{\phiGPquad}[1]{\phi_{GP}^2(z_{#1})}
\newcommand{\PhiGP}[1]{\prod\limits_{#1 = 1}^N \phiGP{#1}}
\newcommand{\PhiGPQuad}[1]{\prod\limits_{#1 = 1}^N \phiGPquad{#1}}
\newcommand{\BrPhiGP}[1]{\prod\limits_{#1 = 1}^N \br{#1} \phiGP{#1}}
\newcommand{\BrPhiGPQuad}[1]{\prod\limits_{#1 = 1}^N \brquad{#1} \phiGPquad{#1}}
%\newcommand{\bmx}[1]{\bm{x}_{#1}}
\newcommand{\bmxs}{\bm{x}'}
%\newcommand{\bmxp}{\bm{x}^{\perp}}
\newcommand{\bmxps}{\bm{x}'^{\perp}}
\newcommand{\bmyp}{\bm{y}^{\perp}}
\newcommand{\bmXp}[1]{\bm{x}^{\perp}_{#1}}
\newcommand{\bmYp}[1]{\bm{y}^{\perp}_{#1}}

\newcommand{\Sum}[1]{\sum\limits_{#1=1}^N}
\newcommand{\Summ}[3]{\sum\limits_{#1 = #2}^{#3}}
\newcommand{\Prod}[1]{\prod\limits_{#1=1}^N}
\newcommand{\Nabla}[1]{\nabla_{#1}}
\newcommand{\NablaPerp}[1]{\nabla_{#1}^{\perp}}
%\newcommand{\laplace}{\mathop{}\!\mathbin\bigtriangleup}
\newcommand{\Laplace}[1]{\laplace_{#1}}
\newcommand{\SumLaplace}[1]{\sum\limits_{#1=1}^N  \laplace_{#1}}
\newcommand{\SumNabla}[1]{\sum\limits_{#1=1}^N \nabla_{#1}}
\newcommand{\SumLaplacePerp}[1]{\sum\limits_{#1=1}^N  \laplace_{#1}^{\perp}}
\newcommand{\SumLaplaceEindim}[1]{\sum\limits_{#1=1}^N \partial_{#1}^2}
\newcommand{\Hdimdreifull}{ - \SumLaplace{j} + V_r^{\perp} + V_L
  + \sum\limits_{1 \le i<j \le N} v_a(|\bm{x}_i - \bm{x}_j|)}
\newcommand{\WW}[2]{v_a(|\bm{x}_#1 - \bm{x}_#2|)}
\newcommand{\WWsum}[2]{\sum\limits_{1 \le #1 < #2 \le N} v_a(|\bm{x}_#1 - \bm{x}_#2|)}
\newcommand{\WWsumDelta}[2]{\sum\limits_{1 \le #1 < #2 \le N} \delta(z_#1 - z_#2)}
\newcommand{\WWsumOmega}[1]{\sum\limits_{1 \le #1 \le N} \delta(z - z_#1^{\omega})}
\newcommand{\EGPN}{E^{\text{GP}}(N,L,g)}
\newcommand{\EGPgamma}{E^{\text{GP} , \omega}_N}
\newcommand{\xperp}{\bm{x}^{\perp}}
\newcommand{\Xperp}{\bm{X}^{\perp}}
\newcommand{\xperps}{\bm{x'}^{\perp}}
\newcommand{\Xperps}{\bm{X'}^{\perp}}
\newcommand{\AnfDi}{\overline{\rho}}
\newcommand{\Ngmu}{N_{g_N, \mu_N}}
\newcommand{\Ngmuj}{N_{g_N, \mu_N}\left( \lintv{p} \right)}
\newcommand{\widehatNgmu}{\widehat  N_{g_N, \mu_N}}
\newcommand{\HLS}{H_{\text{L.S.}}^{1}}
\newcommand{\HLSO}{H_{\text{L.S.}}^{1,\omega}}
\newcommand{\HLSN}{H_{\text{L.S.},N}^{\omega}}


%\newcommand{\E}{\mbox{I\negthinspace E}}
%\DeclareMathOperator{\Var}{Var}

%\newcommand{\E}{\mathds{E}}
%\newcommand{\Var}{\mathrm{Var}}
%\newcommand{\Cov}{\mathrm{Cov}}

\newcommand{\Egr}{E_{0}}
\newcommand{\EgrQM}{E_N^1}
\newcommand{\EGP}{E_{\text{GP}}}
\newcommand{\EGPgammaj}{\EGP^{\gamma,j,\omega}}
\newcommand{\EGPgammajl}{\EGP\left( \gammaNpo \right)}
\newcommand{\EMF}[1]{E_{\text{MF}}^{#1}  (\lintv{p}, \gNpo )}
\newcommand{\EMFiomega}[1]{E^{\text{MF}, #1 , j , \omega}_N}
\newcommand{\EMFj}[1]{E^{\text{MF} #1,\gamma,j,\omega}_N}
\newcommand{\GZEMF}{E_N^{\text{MF}}}
\newcommand{\GZEMFjN}{E_N^{\text{MF},p}}
\newcommand{\GZEMFl}[1]{E_N^{\text{MF}}(\lintv{p},#1)}
\newcommand{\EgrMF}{e^0_{g_N}}
\newcommand{\EangMF}{E_{\text{MF}}^1}
\newcommand{\phiMF}[1]{\phi_N^{\text{MF},#1, p}}
\newcommand{\phiMFIj}[1]{\phi_{\text{MF},\tilde I^{p,\omega}}^{#1}}
\newcommand{\WNP}{W_N^{p,\omega}}
\newcommand{\KphiMF}[1]{\ket{ \phi_{\text{MF}}^{#1} }}
\newcommand{\phiGPonly}{\phi_{\text{GP}}}
\newcommand{\nMF}[1]{n_N^{\text{MF}, #1, j, \omega}}
\newcommand{\nMFIj}[1]{n_{\text{MF},\tilde I^{j,\omega}}^{#1}}
\newcommand{\nQM}[1]{n_N^{#1}}
\newcommand{\nQMli}[1]{\left( n_N^{#1} \right)_{I}}
\newcommand{\nGP}{n_{\text{GP}}^{\gamma}}
\newcommand{\nGPIj}{n_{\text{GP},\tilde I^{j,\omega}}^{\gamma}}
\newcommand{\zintv}[1]{z_{\, N}^{\, #1,\omega}} 
\newcommand{\lintv}[1]{l_{\, N}^{\, #1, \omega}}
\newcommand{\lintvGeord}[1]{l_{\, N, >}^{\, #1, \omega}}
\newcommand{\lintvGeordj}[1]{l_{\, N_j, >}^{\, #1, \omega}}
\newcommand{\lintvGeordjminus}[1]{l_{\, N_{j-1}, >}^{\, #1, \omega}}


\newcommand{\lintvTilde}[1]{\widetilde l_{\, N}^{\, #1,\omega}}
\newcommand{\lintvTildeGeord}[1]{\widetilde l_{\, N, >}^{\, #1,\omega}}
%\newcommand{\lintvgeord}[1]{\tilde l_{\, N}^{\, #1,\omega}} 
\newcommand{\rdm}[1]{ \left( \, #1 \, \right)_N^{(1)} }

\def\C{\mathbbm C}
\def\Z{\mathbbm Z}
\def\R{{\mathbbm R}}
\def\N{\mathbbm N}

\end{comment}

\newcommand{\rhodm}{\mathscr D}
\newcommand{\rhodmGCE}{\rhodm_{\text{gce}}(\beta,\mu)}

\newcommand{\lintvGeordjminus}[1]{l_{\, N_{j-1}, >}^{\, #1, \omega}}

\newcommand{\lintvGeordj}[1]{l_{\, N_j, >}^{\, #1, \omega}}


\newcommand{\hMF}{\hamopein_N^{\text{MF}}}
\newcommand{\hMFjN}{\hamopein_N^{\text{MF},j}}
\newcommand{\hMFjgN}{\hamopein^{\text{MF}}(\lintv{p}, \gNpo)}
\newcommand{\hMFi}{\hamopein_{\text{MF}}^{\gamma_N^{p,\omega},(i)}}
%\newcommand{\hMFi}{\hamopein^{\text{MF},i}_N}
\newcommand{\hMFNgl}{\hamopein_N^{\text{MF}}(\gamma_N^{p,\omega})}
\newcommand{\hMFiomega}{\hamopein^{\text{MF}, i , \omega}_N}
\newcommand{\hMFomega}{\hamopein^{\text{MF}}_N}
\newcommand{\hMFiteTeilchen}{\hamopein^{\text{MF}, (i)}_{N}}
\newcommand{\hMFjteTeilchenNgo}{\hamopein^{\text{MF}, (j)}(\lintv{p}, N_N^p g_N)}
\newcommand{\hMFpNjteTeilchen}{\hamopein^{\text{MF}, p, (j)}_{N}}
\newcommand{\hamopein}{h}
\newcommand{\hamopN}{\hamop{N}}
\newcommand{\hamoptildeN}{\hamop{\widetilde N}}
\newcommand{\hamoptildeNLambda}{\hamopLambda{\widetilde N}}
\newcommand{\hamoptildeNLambdaN}{\hamopLambdaN{\widetilde N}}
\newcommand{\hamopNomega}{\hamop{N}^{\omega}}
\newcommand{\hamopNiomega}{H_{N}^{i,\omega}}
\newcommand{\hamopNjomega}{H_{N}^{j}}
\newcommand{\hamopeinL}{h_L}
\newcommand{\hamopL}{H_L}
\newcommand{\hamop}[1]{\mathcal H^{(#1)}}
%\newcommand{\hamopLambda}[1]{\mathcal H^{(#1)}_{\domain}
\newcommand{\hamopLambda}[1]{\mathcal H^{(#1)}_{\Lambda}}
\newcommand{\hamopLambdaN}[1]{\mathcal H^{(#1)}_{\Lambda_N}}
\newcommand{\hamopNganz}[1]{\mathcal H^{\otimes #1}}
\newcommand{\sym}{\text{sym}}
\newcommand{\fock}{\mathcal F}
\newcommand{\fockL}{\mathcal F_L}
\newcommand{\fockH}{\fock(\hil)}
\newcommand{\fockN}{\bigoplus\limits_{N=0}^{\infty} \NTeilchenhil}
\newcommand{\fockHL}{\fockL(\hilL)}
\newcommand{\fockNL}{\bigoplus\limits_{N=0}^{\infty} \NTeilchenhil_L}
\newcommand{\focksymN}{\bigoplus\limits_{N=0}^{\infty} \NTeilchenhilsym}
\newcommand{\focksymtildeN}{\bigoplus\limits_{\widetilde N=0}^{\infty} \mathscr{H}^{(\widetilde N), \text{sym}}_{\Lambda_N}}
\newcommand{\fockNskalar}[2]{\sum\limits_{N=0}^{\infty} \langle \,#1\, | \,#2\, 
\rangle_{\NTeilchenhil}}
\newcommand{\focksymNskalar}[2]{\sum\limits_{N=0}^{\infty} \langle \,#1\, | 
\,#2\, \rangle_{\NTeilchenhilsym}}
\newcommand{\skalarcd}{\langle \, \cdot \, | \, \cdot \, \rangle}
\newcommand{\fockNskalarcd}{\fockNskalar{\,\cdot\,}{\,\cdot\,}}
\newcommand{\focksymNskalarcd}{\focksymNskalar{\cdot}{\cdot}}
\newcommand{\fockNnorm}[1]{\|#1\|_{\fockN}}
\newcommand{\focksymNnorm}[1]{\|#1\|_{\focksymN}}
\newcommand{\fockNnormcd}{\|\,\cdot\,\|_{\fockN}}
\newcommand{\focksymNnormcd}{\|\,\cdot\,\|_{\focksymN}}
\newcommand{\fockhilNnorm}[1]{\sum\limits_{N=0}^{\infty} \hilNnorm{#1}^2}
\newcommand{\focksymhilNnorm}[1]{\sum\limits_{N=0}^{\infty} \hilNsymnorm{#1}^2}
\newcommand{\fockhilNnormw}[1]{\left(\sum\limits_{N=0}^{\infty} 
\hilNnorm{#1}^2 \right)^{\frac{1}{2}}}
\newcommand{\focksym}{\mathcal F^{\, \text{sym}}_{\Lambda_N}}
\newcommand{\focksymh}{\mathcal F_{\text{sym}}(\hil)}
\newcommand{\focksymskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\mathcal F^{\, \text{sym}}_{\Lambda_N}}}
\newcommand{\focksymskalarcd}{\focksymskalar{\cdot}{\cdot}}
\newcommand{\EinTeilchenhil}{\mathscr H^{(1)}}
\newcommand{\EinTeilchenhilLambda}{\mathscr H^{(1)}_{\Lambda}}
\newcommand{\EinTeilchenhilLambdaN}{\mathscr H^{(1)}_{\Lambda_N}}
\newcommand{\NTeilchenhil}{\mathscr H^{(N)}}
\newcommand{\NTeilchenhilLambda}{\mathscr H^{(N)}_{\Lambda}}
\newcommand{\NtildeTeilchenhil}{\mathscr H^{(\widetilde N)}}
\newcommand{\NtildeTeilchenhilLambda}{\mathscr H^{(\widetilde N)}_{\Lambda}}
\newcommand{\NtildeTeilchenhilLambdaN}{\mathscr H^{(\widetilde N)}_{\Lambda_N}}
\newcommand{\XTeilchenhil}[1]{\mathscr H^{(#1)}}
\newcommand{\XTeilchenhilLambda}[1]{\mathscr H^{(#1)}_{\Lambda}}
\newcommand{\XTeilchenhilLambdaN}[1]{\mathscr H^{(#1)}_{\Lambda_N}}
\newcommand{\XteilchenhilNp}[1]{\mathscr H^{(#1)}_{N,p}}
\newcommand{\XTeilchenhilomega}[1]{\mathscr H^{(#1),\omega}}
\newcommand{\XTeilchenhilsym}[1]{\mathscr H^{(#1)}_{\sym}}
\newcommand{\XTeilchenhilsymLambda}[1]{\mathscr H^{(#1),\sym}_{\Lambda}}
\newcommand{\XTeilchenhilsymLambdaN}[1]{\mathscr H^{(#1),\sym}_{\Lambda_N}}
\newcommand{\XTeilchenhilsymp}[1]{\mathscr H^{(#1)}_{N, p, \sym}}
\newcommand{\XTeilchenhilsymN}[1]{\mathscr H^{(#1)}_{N, \sym}}
\newcommand{\NTeilchenhilsym}{\NTeilchenhil_{\text{sym}}}
\newcommand{\NTeilchenhilsymLambda}{\mathscr H^{(N), \text{sym}}_{\Lambda}}
\newcommand{\NtildeTeilchenhilsym}{\NtildeTeilchenhil_{\text{sym}}}
\newcommand{\NtildeTeilchenhilsymLambda}{\mathscr H^{(\widetilde N), \text{sym}}_{\Lambda}}
\newcommand{\NtildeTeilchenhilsymLambdaN}{\mathscr H^{(\widetilde N), \text{sym}}_{\Lambda_N}}
\newcommand{\NTeilchenhilskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\NTeilchenhil}}
\newcommand{\XTeilchenhilskalar}[3]{\langle \, #2 \, | \, #3 \, 
\rangle_{\XTeilchenhil{#1}}}
\newcommand{\XTeilchenhilskalarcd}[1]{\langle \, \cdot \, | \, \cdot \, 
\rangle_{\XTeilchenhil{#1}}}
\newcommand{\XTeilchenhilnorm}[2]{ \| #2 \|_{\XTeilchenhil{#1}}}
\newcommand{\XTeilchenhilNsymorm}[2]{ \| #2 \|_{\XTeilchenhilsym{#1}}}
\newcommand{\NTeilchenhilsymskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\NTeilchenhilsym}}
\newcommand{\NtildeTeilchenhilsymskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\NtildeTeilchenhilsym}}
\newcommand{\NtildeTeilchenhilsymskalarLambda}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{\NtildeTeilchenhilsymLambdaN}}
\newcommand{\NTeilchenhilskalarcd}{\NTeilchenhilskalar{\cdot}{\cdot}}
\newcommand{\NTeilchenhilsymskalarcd}{\NTeilchenhilsymskalar{\cdot}{\cdot}}
\newcommand{\NtildeTeilchenhilsymskalarcd}{\NtildeTeilchenhilsymskalar{\cdot}{\cdot}}
\newcommand{\NtildeTeilchenhilsymskalarcdLambda}{\NtildeTeilchenhilsymskalarLambda{\cdot}{\cdot}}
\newcommand{\Lskalar}[2]{\langle \, #1 \, | \, #2 \, 
\rangle_{L^2(\mathds R^{Nd},\mathds C)}}
\newcommand{\Lskalarcd}{\Lskalar{\cdot}{\cdot}}
\newcommand{\NTeilchenhilnorm}[1]{\| #1 \|_{\NTeilchenhil}}
\newcommand{\NTeilchenhilnormcd}{\| \cdot \|_{\NTeilchenhil}}
\newcommand{\HsymN}{\mathscr{H}_{\text{sym}}^{(N)}}
\newcommand{\skalar}[2]{\langle #1, #2 \rangle}
\newcommand{\Nskalar}[2]{\sum\limits_{N=0}^{\infty} \langle 
        #1^{(N)} | #2^{(N)} \rangle_{\mathscr{H}_{\text{sym}}^{(N)}}}
\newcommand{\nskalar}[2]{\langle 
        #1^{(N)} | #2^{(N)} \rangle_{\mathscr{H}_{\text{sym}}^ {(N)}}}        
\newcommand{\fockskalar}[2]{\langle #1 | #2 \rangle_{\fock}}
\newcommand{\fockHskalar}[2]{\langle #1 | #2 \rangle_{\fockH}}
\newcommand{\focknorm}[1]{\|#1\|_{\fock}}
\newcommand{\EskalarZ}[2]{\langle #1 | #2 \rangle_{\mathcal E}}
\newcommand{\EskalarS}[6]{\langle #1 \otimes #2 \otimes \ldots \otimes #3, #4 
\otimes #5\otimes \ldots \otimes #6 \rangle_{\mathcal E}}
\newcommand{\Hskalar}[3]{\langle #1_{#3} | #2_{#3} \rangle_{\mathscr{H}_{#3}}}
\newcommand{\hil}{\mathscr{H}}
\newcommand{\hilL}{\mathscr{H_L}}
\newcommand{\hilN}{\hil^{(N)}}
\newcommand{\hilNganz}{\hil^{\otimes N}}
\newcommand{\hilX}[1]{\hil_{#1}}
\newcommand{\hilNsym}{\hil^{(N)}_{\sym}}
\newcommand{\hilNtildesym}{\hil^{(\widetilde N)}_{\sym}}
\newcommand{\hilNtildesymLambda}{\hil^{(\widetilde N),\text{sym}}_{\Lambda}}
\newcommand{\hilNtildesymLambdaN}{\hil^{(\widetilde N),\text{sym}}_{\Lambda_N}}
\newcommand{\hilskalar}[2]{\langle \,#1\, | \,#2\, \rangle_{\hil}}
\newcommand{\hilskalarcd}{\hilskalar{\cdot}{\cdot}}
\newcommand{\hilNskalar}[2]{\langle \,#1\, | \,#2\, \rangle_{\hilN}}
\newcommand{\hilXskalar}[3]{\langle \,#1\, | \,#2\, \rangle_{\mathscr{H}_{#3}}}
\newcommand{\hilNsymskalar}[2]{\langle \, #1 \,  | \, #2 \, \rangle_{\hilNsym}}
\newcommand{\hilNskalarcd}{\hilNskalar{\,\cdot\,}{\,\cdot\,}}
\newcommand{\hilNsymskalarcd}{\hilNsymskalar{\,\cdot\,}{\,\cdot}}
\newcommand{\hilnorm}[1]{\|\, #1\, \|_{\hil}}
\newcommand{\hilNnorm}[1]{\|\, #1\, \|_{\hilN}}
\newcommand{\hilNsymnorm}[1]{\|\, #1\, \|_{\hilNsym}}
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ket}[1]{| #1 \rangle}
\newcommand{\braket}[2]{\langle #1 , #2 \rangle}
%\newcommand{\braketop}[3]{\, \left\langle #1 \,|\, #2 \,|\, #3 \,\right\rangle}
%\newcommand{\braketop}[3]{\langle #1 |\, #2 \,| #3 \rangle}
\newcommand{\projec}[1]{\ket{#1}\bra{#1}}
\newcommand{\ONB}[1]{\left\{ \phi_{#1} \right\}_{#1 \in \mathds N}}
\newcommand{\ONBN}[1]{\left\{ \phi_{#1_1} \otimes \phi_{#1_2} \otimes \ldots \otimes \phi_{#1_N} \right\}_{#1_1, #1_2, \ldots, #1_N \in \mathds N}}

\newcommand{\gNpo}{N_N^p g_N}
\newcommand{\gNpotilde}{\widetilde g_N^{\,p}}
\newcommand{\gammaNpo}{\gamma_N^{\,p}}
\newcommand{\gammaNpotilde}{\widetilde \gamma_N^{\,p}}

\newcommand{\NNpGeord}[1]{N_{N,>}^{#1}}

\newcommand{\EQM}[1]{E_{\text{QM}}^{#1}\left( \widetilde N_N^p, \lintv{p}, g_N \right)}
\newcommand{\phiQM}[1]{\phi_N^{#1}}
\newcommand{\Hdimdrei}{H_{3D}(N,L,r,a)}
\newcommand{\br}[1]{b_r(\bm{x}^{\perp}_{#1})}
\newcommand{\Br}[1]{\prod\limits_{#1 = 1}^N \br{#1}}
\newcommand{\brquad}[1]{b_r^2(\bm{x}^{\perp}_{#1})}
\newcommand{\BrQuad}[1]{\prod\limits_{#1 = 1}^N \brquad{#1}}
\newcommand{\phigp}{\phi_{\text{GP}}}
\newcommand{\phigpgamma}{\phi_{\text{GP}}^{g_N}}
\newcommand{\phigpgNp}{\phi_{\text{GP}}(N_N^p, \lintv{p}, g_N)}
\newcommand{\phigpgeinsp}{\phi_{\text{GP}}(1, \lintv{p}, N_N^p g_N)}
\newcommand{\phigpgammap}{\phi_{\text{GP}}^{1, \gammaNpo}}
\newcommand{\phigpgNpo}{\phi_{\text{GP}}^{\lintv{p}, \gNpo}}
\newcommand{\phigpgammapeinslg}{\phi_{\text{GP}}(1, \lintv{p}, N_N^p g_N)}
\newcommand{\EGPgammaNpo}{\EGP ( 1, 1, \gammaNpo )}
\newcommand{\EGPgNpo}{\EGP(1, \lintv{p}, \gNpo)}
\newcommand{\phigpgammaptilde}{\widetilde\phi_{\text{GP}}^{\gammaNpo}}
\newcommand{\phigpgNpotilde}{\widetilde\phi_{\text{GP}}^{\, \lintv{p}, \gNpo}}
\newcommand{\phigpgammapl}{\phi_N^{\text{GP}}(\gamma_N^{p,\omega})}
\newcommand{\phigpgammaIp}{\phi_{\text{GP}, I^{p,\omega}}^{\gamma}}
\newcommand{\Kphigp}{\ket{\phi_{\text{GP}}}}
\newcommand{\Kphigpgamma}{\ket{\phi_N^{\text{GP}}}}
\newcommand{\Kphigpgammap}{\ket{\phi_{\text{GP}, I^{p,\omega}}^{\gamma}}}
\newcommand{\phigpN}{\phi_{\text{GP}}^{\otimes N}}
\newcommand{\phigpNjomega}{\left( \phigpgammap \right)^{\otimes N_N^p}}
\newcommand{\phiGP}[1]{\phi_{GP}(z_{#1})}
\newcommand{\phiGPL}[1]{\phi_{GP}\left( z_{#1}/L \right)}
\newcommand{\phiGPz}{\phi_{GP}(z)}
\newcommand{\phiGPzs}{\phi_{GP}(z')}
\newcommand{\phiGPquad}[1]{\phi_{GP}^2(z_{#1})}
\newcommand{\PhiGP}[1]{\prod\limits_{#1 = 1}^N \phiGP{#1}}
\newcommand{\PhiGPQuad}[1]{\prod\limits_{#1 = 1}^N \phiGPquad{#1}}
\newcommand{\BrPhiGP}[1]{\prod\limits_{#1 = 1}^N \br{#1} \phiGP{#1}}
\newcommand{\BrPhiGPQuad}[1]{\prod\limits_{#1 = 1}^N \brquad{#1} \phiGPquad{#1}}
\newcommand{\bmx}[1]{\bm{x}_{#1}}
\newcommand{\bmxs}{\bm{x}'}
\newcommand{\bmxp}{\bm{x}^{\perp}}
\newcommand{\bmxps}{\bm{x}'^{\perp}}
\newcommand{\bmyp}{\bm{y}^{\perp}}
\newcommand{\bmXp}[1]{\bm{x}^{\perp}_{#1}}
\newcommand{\bmYp}[1]{\bm{y}^{\perp}_{#1}}

\newcommand{\Sum}[1]{\sum\limits_{#1=1}^N}
\newcommand{\Summ}[3]{\sum\limits_{#1 = #2}^{#3}}
\newcommand{\Prod}[1]{\prod\limits_{#1=1}^N}
\newcommand{\Nabla}[1]{\nabla_{#1}}
\newcommand{\NablaPerp}[1]{\nabla_{#1}^{\perp}}
\newcommand{\laplace}{\mathop{}\!\mathbin\bigtriangleup}
\newcommand{\Laplace}[1]{\laplace_{#1}}
\newcommand{\Dlaplace}[1]{\laplace_{#1}^{\mathrm{D}}}
\newcommand{\Nlaplace}[1]{\laplace_{#1}^{\text{Nm}}}
\newcommand{\SumLaplace}[1]{\sum\limits_{#1=1}^N  \laplace_{#1}}
\newcommand{\SumNabla}[1]{\sum\limits_{#1=1}^N \nabla_{#1}}
\newcommand{\SumLaplacePerp}[1]{\sum\limits_{#1=1}^N  \laplace_{#1}^{\perp}}
\newcommand{\SumLaplaceEindim}[1]{\sum\limits_{#1=1}^N \partial_{#1}^2}
\newcommand{\Hdimdreifull}{ - \SumLaplace{j} + V_r^{\perp} + V_L
  + \sum\limits_{1 \le i<j \le N} v_a(|\bm{x}_i - \bm{x}_j|)}
\newcommand{\WW}[2]{v_a(|\bm{x}_#1 - \bm{x}_#2|)}
\newcommand{\WWsum}[2]{\sum\limits_{1 \le #1 < #2 \le N} v_a(|\bm{x}_#1 - \bm{x}_#2|)}
\newcommand{\WWsumDelta}[2]{\sum\limits_{1 \le #1 < #2 \le N} \delta(z_#1 - z_#2)}
\newcommand{\WWsumOmega}[1]{\sum\limits_{1 \le #1 \le N} \delta(z - z_#1^{\omega})}
\newcommand{\EGPN}{E^{\text{GP}}(N,L,g)}
\newcommand{\EGPgamma}{E^{\text{GP} , \omega}_N}
\newcommand{\xperp}{\bm{x}^{\perp}}
\newcommand{\Xperp}{\bm{X}^{\perp}}
\newcommand{\xperps}{\bm{x'}^{\perp}}
\newcommand{\Xperps}{\bm{X'}^{\perp}}
\newcommand{\AnfDi}{\overline{\rho}}
\newcommand{\Ngmu}{N_{g_N, \mu_N}}
\newcommand{\Ngmuj}{N_{g_N, \mu_N}\left( \lintv{p} \right)}
\newcommand{\widehatNgmu}{\widehat  N_{g_N, \mu_N}}

\newcommand{\cutofffunctioneins}[2]{\chi_{#1,#2}}
\newcommand{\cutofffunctionzwei}[2]{\widetilde \chi_{#1,#2}}
\newcommand{\cutofffunctiondrei}[2]{\widehat \chi_{#1,#2}}


\newcommand{\Heinsomega}{\mathcal H_{N}^{\text{D}, \omega}}
\newcommand{\HeinsomegaLS}{\mathcal H_{N, \infty}^{\text{D}, \omega}}
\newcommand{\WidetildeHeinsomegaLS}{\widetilde{\mathcal H}_{N, \infty}^{\text{D}, \omega}}


%\newcommand{\E}{\mbox{I\negthinspace E}}
%\DeclareMathOperator{\usepackage{graphicx}
% \usepackage{german}
%\usepackage[bookmarks]{hyperref}
\usepackage{amssymb}

\newcommand{\E}{\mathds{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

\newcommand{\Egr}{E_{0}}
\newcommand{\EgrQM}{E_N^1}
\newcommand{\EGP}{E_{\text{GP}}}
\newcommand{\EGPgammaj}{\EGP^{\gamma,j,\omega}}
\newcommand{\EGPgammajl}{\EGP\left( \gammaNpo \right)}
\newcommand{\EMF}[1]{E_{\text{MF}}^{#1}  (\lintv{p}, \gNpo )}
\newcommand{\EMFiomega}[1]{E^{\text{MF}, #1 , j , \omega}_N}
\newcommand{\EMFj}[1]{E^{\text{MF} #1,\gamma,j,\omega}_N}
\newcommand{\GZEMF}{E_N^{\text{MF}}}
\newcommand{\GZEMFjN}{E_N^{\text{MF},p}}
\newcommand{\GZEMFl}[1]{E_N^{\text{MF}}(\lintv{p},#1)}
\newcommand{\EgrMF}{e^0_{g_N}}
\newcommand{\EangMF}{E_{\text{MF}}^1}
\newcommand{\phiMF}[1]{\phi_N^{\text{MF},#1, p}}
\newcommand{\phiMFIj}[1]{\phi_{\text{MF},\tilde I^{p,\omega}}^{#1}}
\newcommand{\WNP}{W_N^{p,\omega}}
\newcommand{\KphiMF}[1]{\ket{ \phi_{\text{MF}}^{#1} }}
\newcommand{\phiGPonly}{\phi_{\text{GP}}}
\newcommand{\nMF}[1]{n_N^{\text{MF}, #1, j, \omega}}
\newcommand{\nMFIj}[1]{n_{\text{MF},\tilde I^{j,\omega}}^{#1}}
\newcommand{\nQM}[1]{n_N^{#1}}
\newcommand{\nQMli}[1]{\left( n_N^{#1} \right)_{I}}
\newcommand{\nGP}{n_{\text{GP}}^{\gamma}}
\newcommand{\nGPIj}{n_{\text{GP},\tilde I^{j,\omega}}^{\gamma}}
\newcommand{\zintv}[1]{z_{N}^{#1,\omega}} 
\newcommand{\lintv}[1]{l_{N}^{(#1), \omega}}
\newcommand{\lintvGeord}[1]{l_{N, >}^{(#1), \omega}}
\newcommand{\lintvGeordM}[1]{l_{\, M, >}^{\, #1, \omega}}
\newcommand{\lintvTilde}[1]{\widetilde l_{\, M}^{\, #1,\omega}}
\newcommand{\lintvTildeGeord}[1]{\widetilde l_{\, N, >}^{\, #1,\omega}}
%\newcommand{\lintvgeord}[1]{\tilde l_{\, N}^{\, #1,\omega}} 
\newcommand{\rdm}[1]{ \left( \, #1 \, \right)_N^{(1)} }

\newcommand{\nuN}{\nu_N}
\newcommand{\gN}{g_N}
\newcommand{\muN}{\mu_N}
\newcommand{\xiN}{\xi_N}
\newcommand{\lambdaN}{\lambda_N}
\newcommand{\LN}{L_N}
\newcommand{\llargest}{l_{N,>}^{\, (1),\omega}}
\newcommand{\ljomega}{l^{j,\omega}}
\newcommand{\lNjomega}{l_N^{j, \omega}}
\newcommand{\tildelNjomega}{\tilde l_N^{j, \omega}}
\newcommand{\WNjomega}{W_N^{j , \omega}}
\newcommand{\llargestLambda}{l_{\Lambda,>}^{(1)}}
\newcommand{\llargestLambdaZwei}{l_{\Lambda,>}^{(2)}}
\newcommand{\llargestzwei}{l_{N,>}^{\, (2),\omega}}
\newcommand{\llargestfunf}{l_{N,>}^{\, (5),\omega}}
\newcommand{\llargesttilde}{\tilde l_{N,>}^{\, (1),\omega}}
\newcommand{\llargesttildezwei}{\tilde l_{N,>}^{\, (2),\omega}}
\newcommand{\llargesttildek}{\tilde l_{k,>}^{\, (1),\omega}}
\newcommand{\llargesthatk}{\hat l_{k,>}^{\, (1),\omega}}
\newcommand{\llargesttildezweik}{\tilde l_{k,>}^{\, (2),\omega}}
\newcommand{\llargesthatzweik}{\hat l_{k,>}^{\, (2),\omega}}
\newcommand{\Mlargest}{M_{N,>}^{(1)}}
\newcommand{\Mlargestomega}{M_{N,>}^{(1),\omega}}
\newcommand{\MlargestLambda}{M_{\Lambda,>}^{(1)}}
\newcommand{\Nlargest}{N_{N,>}^{(1)}}
\newcommand{\Nlargestomega}{N_{N,>}^{(1),\omega}}
\newcommand{\lj}{l_N^j}
\newcommand{\ljLambda}{l_{\Lambda}^{j}}
\newcommand{\hatlj}{\hat l^{(j),\omega}}
\newcommand{\nMjgz}{n_{M_{\Lambda}^{j}}}

\newcommand{\domain}{\Lambda}

\newcommand{\ceins}{c_1}
\newcommand{\czwei}{c_2}
\newcommand{\Lzwei}{L^2}

\newcommand{\ELSomega}{E_{\mathrm{LS}}^{1,\omega}}
\newcommand{\EQMomega}{E^{1,\omega}_{\mathrm{QM}}}
\newcommand{\ELS}{E_{\mathrm{LS}}^{1}}
\newcommand{\ezwei}{e^2}

\newcommand{\tildeWNjomega}{\widetilde W_N^{j,\omega}}
\newcommand{\tildeljomega}{\tilde l_N^{j,\omega}}
\newcommand{\ParticleNumberInLargestInterval}{\widetilde N_{N,>}^{(1),\omega}}
\newcommand{\nMjLambdaj}{n_{M^{j}_{\Lambda}}^{j}}
\newcommand{\MNjomega}{M^{j,\omega}_{N}}
\newcommand{\hatMNjomega}{\hat M^{j,\omega}_{N}}
\newcommand{\cdrei}{c_3}



%---------------------------------------------------------------------

%\DeclareMathOperator{\tr}{tr}
%\pagestyle{headings} % einf\"{u}gen einer Kopfzeile
% \includeonly{kap2} % nur das 2.Kapitel wird compiliert
%\geometry



